Bad Foundations and Manipulable Objects

Imagine a student -- let's call him `E', and make him a "he" -- that is enrolled in Calculus 2, and who believes that to pass in maths courses he only needs to memorize methods and apply them quickly and without errors. Let's imagine that `E' is an `E'xtreme case of "bad foundations" and that he knows how to solve $x+2=5$ by doing $x=5-2=3$, but he doesn't know how to substitute the $x$ in $x+2=5$ by 3, and the only way that he knows of "testing the solution" is to apply the same method again and check that he got the same result. When we are teaching Calculus to classes that have many students that are extreme cases of bad foundations we need new strategies and tools; for example, we can't pretend that "taking a particular case" is an obvious operation anymore -- instead we need ways to make these operations easy to visualize. This article shows a way to do that using Maxima.

==> edrx21chars-d.tex <==
% This file:
%   http://angg.twu.net/LATEX/edrx21chars-d.tex.html
%   http://angg.twu.net/LATEX/edrx21chars-d.tex
%           (find-angg "LATEX/edrx21chars-d.tex")
% Author: Eduardo Ochs <eduardoochs@gmail.com>
% Version: 2021dec11 (?)
% Public domain.
%
% This file contains the "definitions in pdflatex" for the unicode
% characters listed here:
%
%                        (find-eev "eev-compose-hash.el"    "unicode-characters")
%   http://angg.twu.net/eev-current/eev-compose-hash.el.html#unicode-characters
%
% The "definitions in lualatex" for the same characters are in this
% other file:
%
%                (find-LATEX "edrx21chars.tex")
%   http://angg.twu.net/LATEX/edrx21chars.tex.html
%   http://angg.twu.net/LATEX/edrx21chars.tex
%
% There is a test here:
%
%                (find-LATEX "2021composes-hash.tex")
%   http://angg.twu.net/LATEX/2021composes-hash.tex.html
%   http://angg.twu.net/LATEX/2021composes-hash.tex
%
% The "\DeclareUnicodeCharacter..."s below are generated by executing
% some sexps in Emacs and then copying their output from a temporary
% buffer to this file.
%
% This file: (find-LATEX "edrx21chars-d.tex")
%   Variant: (find-LATEX "edrx21chars.tex")
%  Based on: (find-LATEX "edrxchars.tex")
%            (find-LATEX "edrx15chars.tex")
%            (find-LATEX "edrx20chars.tex")
%            (find-LATEX "2019oxford-chars.tex")
%       Gen: (find-eev "eev-compose-hash.el")
%            (find-estring (ee-composes-to-declareunicodes))
%       See: (find-LATEX "2021composes-hash.tex")


\DeclareUnicodeCharacter{00A1}{\text{\textexclamdown}} % ¡
\DeclareUnicodeCharacter{00A7}{\S}                 % §
\DeclareUnicodeCharacter{00AC}{\neg}               % ¬
\DeclareUnicodeCharacter{00B0}{^\circ}             % °
\DeclareUnicodeCharacter{00B1}{\pm}                % ±
\DeclareUnicodeCharacter{00B2}{\superscriptTwo}    % ²
\DeclareUnicodeCharacter{00B3}{\superscriptThree}  % ³
\DeclareUnicodeCharacter{00B7}{\cdot}              % ·
\DeclareUnicodeCharacter{00B9}{\superscriptOne}    % ¹
\DeclareUnicodeCharacter{00D7}{\times}             % ×
\DeclareUnicodeCharacter{00F7}{\div}               % ÷
\DeclareUnicodeCharacter{0393}{\Gamma}             % Γ
\DeclareUnicodeCharacter{0394}{\Delta}             % Δ
\DeclareUnicodeCharacter{0398}{\Theta}             % Θ
\DeclareUnicodeCharacter{039B}{\Lambda}            % Λ
\DeclareUnicodeCharacter{03A0}{\Pi}                % Π
\DeclareUnicodeCharacter{03A3}{\Sigma}             % Σ
\DeclareUnicodeCharacter{03A6}{\Phi}               % Φ
\DeclareUnicodeCharacter{03A8}{\Psi}               % Ψ
\DeclareUnicodeCharacter{03A9}{\Omega}             % Ω
\DeclareUnicodeCharacter{03B1}{\alpha}             % α
\DeclareUnicodeCharacter{03B2}{\beta}              % β
\DeclareUnicodeCharacter{03B3}{\gamma}             % γ
\DeclareUnicodeCharacter{03B4}{\delta}             % δ
\DeclareUnicodeCharacter{03B5}{\varepsilon}        % ε
\DeclareUnicodeCharacter{03B6}{\zeta}              % ζ
\DeclareUnicodeCharacter{03B7}{\eta}               % η
\DeclareUnicodeCharacter{03B8}{\theta}             % θ
\DeclareUnicodeCharacter{03B9}{\iota}              % ι
\DeclareUnicodeCharacter{03BA}{\kappa}             % κ
\DeclareUnicodeCharacter{03BB}{\lambda}            % λ
\DeclareUnicodeCharacter{03BB}{\ensuremath{\lambda}}            % λ
\DeclareUnicodeCharacter{03BC}{\mu}                % μ
\DeclareUnicodeCharacter{03BD}{\nu}                % ν
\DeclareUnicodeCharacter{03BE}{\xi}                % ξ
\DeclareUnicodeCharacter{03C0}{\pi}                % π
\DeclareUnicodeCharacter{03C1}{\rho}               % ρ
\DeclareUnicodeCharacter{03C3}{\sigma}             % σ
\DeclareUnicodeCharacter{03C4}{\tau}               % τ
\DeclareUnicodeCharacter{03C6}{\varphi}            % φ
\DeclareUnicodeCharacter{03C7}{\chi}               % χ
\DeclareUnicodeCharacter{03C8}{\psi}               % ψ
\DeclareUnicodeCharacter{03C9}{\omega}             % ω
\DeclareUnicodeCharacter{03D5}{\phi}               % ϕ
\DeclareUnicodeCharacter{1D400}{\mathbf{A}}        % 𝐀
\DeclareUnicodeCharacter{1D401}{\mathbf{B}}        % 𝐁
\DeclareUnicodeCharacter{1D402}{\mathbf{C}}        % 𝐂
\DeclareUnicodeCharacter{1D403}{\mathbf{D}}        % 𝐃
\DeclareUnicodeCharacter{1D404}{\mathbf{E}}        % 𝐄
\DeclareUnicodeCharacter{1D405}{\mathbf{F}}        % 𝐅
\DeclareUnicodeCharacter{1D406}{\mathbf{G}}        % 𝐆
\DeclareUnicodeCharacter{1D407}{\mathbf{H}}        % 𝐇
\DeclareUnicodeCharacter{1D408}{\mathbf{I}}        % 𝐈
\DeclareUnicodeCharacter{1D409}{\mathbf{J}}        % 𝐉
\DeclareUnicodeCharacter{1D40A}{\mathbf{K}}        % 𝐊
\DeclareUnicodeCharacter{1D40B}{\mathbf{L}}        % 𝐋
\DeclareUnicodeCharacter{1D40C}{\mathbf{M}}        % 𝐌
\DeclareUnicodeCharacter{1D40D}{\mathbf{N}}        % 𝐍
\DeclareUnicodeCharacter{1D40E}{\mathbf{O}}        % 𝐎
\DeclareUnicodeCharacter{1D40F}{\mathbf{P}}        % 𝐏
\DeclareUnicodeCharacter{1D410}{\mathbf{Q}}        % 𝐐
\DeclareUnicodeCharacter{1D411}{\mathbf{R}}        % 𝐑
\DeclareUnicodeCharacter{1D412}{\mathbf{S}}        % 𝐒
\DeclareUnicodeCharacter{1D413}{\mathbf{T}}        % 𝐓
\DeclareUnicodeCharacter{1D414}{\mathbf{U}}        % 𝐔
\DeclareUnicodeCharacter{1D415}{\mathbf{V}}        % 𝐕
\DeclareUnicodeCharacter{1D416}{\mathbf{W}}        % 𝐖
\DeclareUnicodeCharacter{1D417}{\mathbf{X}}        % 𝐗
\DeclareUnicodeCharacter{1D418}{\mathbf{Y}}        % 𝐘
\DeclareUnicodeCharacter{1D419}{\mathbf{Z}}        % 𝐙
\DeclareUnicodeCharacter{1D41B}{\mathbf}           % 𝐛
\DeclareUnicodeCharacter{1D422}{\textsl}           % 𝐢
\DeclareUnicodeCharacter{1D42B}{\mathrm}           % 𝐫
\DeclareUnicodeCharacter{1D42C}{\mathsf}           % 𝐬
\DeclareUnicodeCharacter{1D42D}{\text}             % 𝐭
\DeclareUnicodeCharacter{1D4D0}{\mathcal{A}}       % 𝓐
\DeclareUnicodeCharacter{1D4D1}{\mathcal{B}}       % 𝓑
\DeclareUnicodeCharacter{1D4D2}{\mathcal{C}}       % 𝓒
\DeclareUnicodeCharacter{1D4D3}{\mathcal{D}}       % 𝓓
\DeclareUnicodeCharacter{1D4D4}{\mathcal{E}}       % 𝓔
\DeclareUnicodeCharacter{1D4D5}{\mathcal{F}}       % 𝓕
\DeclareUnicodeCharacter{1D4D6}{\mathcal{G}}       % 𝓖
\DeclareUnicodeCharacter{1D4D7}{\mathcal{H}}       % 𝓗
\DeclareUnicodeCharacter{1D4D8}{\mathcal{I}}       % 𝓘
\DeclareUnicodeCharacter{1D4D9}{\mathcal{J}}       % 𝓙
\DeclareUnicodeCharacter{1D4DA}{\mathcal{K}}       % 𝓚
\DeclareUnicodeCharacter{1D4DB}{\mathcal{L}}       % 𝓛
\DeclareUnicodeCharacter{1D4DC}{\mathcal{M}}       % 𝓜
\DeclareUnicodeCharacter{1D4DD}{\mathcal{N}}       % 𝓝
\DeclareUnicodeCharacter{1D4DE}{\mathcal{O}}       % 𝓞
\DeclareUnicodeCharacter{1D4DF}{\mathcal{P}}       % 𝓟
\DeclareUnicodeCharacter{1D4E0}{\mathcal{Q}}       % 𝓠
\DeclareUnicodeCharacter{1D4E1}{\mathcal{R}}       % 𝓡
\DeclareUnicodeCharacter{1D4E2}{\mathcal{S}}       % 𝓢
\DeclareUnicodeCharacter{1D4E3}{\mathcal{T}}       % 𝓣
\DeclareUnicodeCharacter{1D4E4}{\mathcal{U}}       % 𝓤
\DeclareUnicodeCharacter{1D4E5}{\mathcal{V}}       % 𝓥
\DeclareUnicodeCharacter{1D4E6}{\mathcal{W}}       % 𝓦
\DeclareUnicodeCharacter{1D4E7}{\mathcal{X}}       % 𝓧
\DeclareUnicodeCharacter{1D4E8}{\mathcal{Y}}       % 𝓨
\DeclareUnicodeCharacter{1D4E9}{\mathcal{Z}}       % 𝓩
\DeclareUnicodeCharacter{2022}{\bullet}            % •
\DeclareUnicodeCharacter{2026}{\ldots}             % …
\DeclareUnicodeCharacter{2080}{{{}_0}}             % ₀
\DeclareUnicodeCharacter{2081}{{{}_1}}             % ₁
\DeclareUnicodeCharacter{2082}{{{}_2}}             % ₂
\DeclareUnicodeCharacter{2083}{{{}_3}}             % ₃
\DeclareUnicodeCharacter{2084}{{{}_4}}             % ₄
\DeclareUnicodeCharacter{2085}{{{}_5}}             % ₅
\DeclareUnicodeCharacter{2086}{{{}_6}}             % ₆
\DeclareUnicodeCharacter{2087}{{{}_7}}             % ₇
\DeclareUnicodeCharacter{2088}{{{}_8}}             % ₈
\DeclareUnicodeCharacter{2089}{{{}_9}}             % ₉
\DeclareUnicodeCharacter{208A}{{{}_+}}             % ₊
\DeclareUnicodeCharacter{208B}{{{}_-}}             % ₋
\DeclareUnicodeCharacter{208C}{{{}_=}}             % ₌
\DeclareUnicodeCharacter{208D}{{{}_(}}             % ₍
\DeclareUnicodeCharacter{208E}{{{}_)}}             % ₎
\DeclareUnicodeCharacter{2090}{{{}_a}}             % ₐ
\DeclareUnicodeCharacter{2091}{{{}_e}}             % ₑ
\DeclareUnicodeCharacter{2092}{{{}_o}}             % ₒ
\DeclareUnicodeCharacter{2093}{{{}_x}}             % ₓ
\DeclareUnicodeCharacter{2095}{{{}_h}}             % ₕ
\DeclareUnicodeCharacter{2096}{{{}_k}}             % ₖ
\DeclareUnicodeCharacter{2097}{{{}_l}}             % ₗ
\DeclareUnicodeCharacter{2098}{{{}_m}}             % ₘ
\DeclareUnicodeCharacter{2099}{{{}_n}}             % ₙ
\DeclareUnicodeCharacter{209A}{{{}_p}}             % ₚ
\DeclareUnicodeCharacter{209B}{{{}_s}}             % ₛ
\DeclareUnicodeCharacter{209C}{{{}_t}}             % ₜ
\DeclareUnicodeCharacter{2113}{\ell}               % ℓ
\DeclareUnicodeCharacter{214B}{\bindnasrepma}      % ⅋
\DeclareUnicodeCharacter{2190}{\ot}                % ←
\DeclareUnicodeCharacter{2191}{\upto}              % ↑
\DeclareUnicodeCharacter{2192}{\to}                % →
\DeclareUnicodeCharacter{2193}{\dnto}              % ↓
\DeclareUnicodeCharacter{2194}{\bij}               % ↔
\DeclareUnicodeCharacter{2195}{\updownarrow}       % ↕
\DeclareUnicodeCharacter{2196}{\nwarrow}           % ↖
\DeclareUnicodeCharacter{2197}{\nearrow}           % ↗
\DeclareUnicodeCharacter{2198}{\searrow}           % ↘
\DeclareUnicodeCharacter{2199}{\swarrow}           % ↙
\DeclareUnicodeCharacter{21A3}{\epito}             % ↣
\DeclareUnicodeCharacter{21A4}{\mapsfrom}          % ↤
\DeclareUnicodeCharacter{21A6}{\mapsto}            % ↦
\DeclareUnicodeCharacter{21C0}{\rightharpoonup}    % ⇀
\DeclareUnicodeCharacter{21D0}{\Leftarrow}         % ⇐
\DeclareUnicodeCharacter{21D2}{\funto}             % ⇒
\DeclareUnicodeCharacter{21D4}{\Leftrightarrow}    % ⇔
\DeclareUnicodeCharacter{21DD}{\rightsquigarrow}   % ⇝
\DeclareUnicodeCharacter{2200}{\forall}            % ∀
\DeclareUnicodeCharacter{2202}{\partial}           % ∂
\DeclareUnicodeCharacter{2203}{\exists}            % ∃
\DeclareUnicodeCharacter{2205}{\emptyset}          % ∅
\DeclareUnicodeCharacter{2207}{\nabla}             % ∇
\DeclareUnicodeCharacter{2208}{\in}                % ∈
\DeclareUnicodeCharacter{2216}{\backslash}         % ∖
\DeclareUnicodeCharacter{2218}{\circ}              % ∘
\DeclareUnicodeCharacter{221A}{\sqrt}              % √
\DeclareUnicodeCharacter{221E}{\infty}             % ∞
\DeclareUnicodeCharacter{2227}{\land}              % ∧
\DeclareUnicodeCharacter{2228}{\lor}               % ∨
\DeclareUnicodeCharacter{2229}{\cap}               % ∩
\DeclareUnicodeCharacter{222A}{\cup}               % ∪
\DeclareUnicodeCharacter{222B}{\int}               % ∫
\DeclareUnicodeCharacter{223C}{\sim}               % ∼
\DeclareUnicodeCharacter{2243}{\simeq}             % ≃
\DeclareUnicodeCharacter{2245}{\cong}              % ≅
\DeclareUnicodeCharacter{2248}{\approx}            % ≈
\DeclareUnicodeCharacter{2260}{\neq}               % ≠
\DeclareUnicodeCharacter{2261}{\equiv}             % ≡
\DeclareUnicodeCharacter{2264}{\le}                % ≤
\DeclareUnicodeCharacter{2265}{\ge}                % ≥
\DeclareUnicodeCharacter{2282}{\subset}            % ⊂
\DeclareUnicodeCharacter{2283}{\supset}            % ⊃
\DeclareUnicodeCharacter{2286}{\subseteq}          % ⊆
\DeclareUnicodeCharacter{2287}{\supseteq}          % ⊇
\DeclareUnicodeCharacter{2293}{\sqcap}             % ⊓
\DeclareUnicodeCharacter{2294}{\sqcup}             % ⊔
\DeclareUnicodeCharacter{2295}{\oplus}             % ⊕
\DeclareUnicodeCharacter{2296}{\ominus}            % ⊖
\DeclareUnicodeCharacter{2297}{\otimes}            % ⊗
\DeclareUnicodeCharacter{2298}{\oslash}            % ⊘
\DeclareUnicodeCharacter{2299}{\odot}              % ⊙
\DeclareUnicodeCharacter{22A2}{\vdash}             % ⊢
\DeclareUnicodeCharacter{22A3}{\dashv}             % ⊣
\DeclareUnicodeCharacter{22A4}{\top}               % ⊤
\DeclareUnicodeCharacter{22A5}{\bot}               % ⊥
\DeclareUnicodeCharacter{22A8}{\vDash}             % ⊨
\DeclareUnicodeCharacter{22C0}{\bigwedge}          % ⋀
\DeclareUnicodeCharacter{22C1}{\bigvee}            % ⋁
\DeclareUnicodeCharacter{22C2}{\bigcap}            % ⋂
\DeclareUnicodeCharacter{22C3}{\bigcup}            % ⋃
\DeclareUnicodeCharacter{22C4}{\lozenge}           % ⋄
\DeclareUnicodeCharacter{22C5}{\Box}               % ⋅
\DeclareUnicodeCharacter{22EE}{\vdots}             % ⋮
\DeclareUnicodeCharacter{22EF}{\cdots}             % ⋯
\DeclareUnicodeCharacter{2329}{\langle}            % 〈
\DeclareUnicodeCharacter{232A}{\rangle}            % 〉
\DeclareUnicodeCharacter{2581}{\_}                 % ▁
\DeclareUnicodeCharacter{25A1}{\Box}               % □
\DeclareUnicodeCharacter{25FB}{\Box}               % ◻
\DeclareUnicodeCharacter{266D}{\flat}              % ♭
\DeclareUnicodeCharacter{266E}{\natural}           % ♮
\DeclareUnicodeCharacter{266F}{\sharp}             % ♯
\DeclareUnicodeCharacter{27E6}{\llbracket}         % ⟦
\DeclareUnicodeCharacter{27E7}{\rrbracket}         % ⟧
\DeclareUnicodeCharacter{2806}{{:}}                % ⠆

% Local Variables:
% coding: utf-8-unix
% End:



==> edrx21defs.tex <==
% This file: (find-LATEX "edrx21defs.tex")
%       See: (find-LATEX "edrx17defs.tex")
%            (find-LATEX "edrx15defs.tex")
% Loaded by: (find-LATEX "edrx21.sty")
% Version:   2023oct07  <- don't trust this date
%
% Miscellaneous defs, mostly symbols.


% «.categories»			(to "categories")
% «.greek-letters»		(to "greek-letters")
% «.combinators»		(to "combinators")
% «.colors»			(to "colors")
% «.standout»			(to "standout")
% «.mystrut»			(to "mystrut")
% «.bhbox»			(to "bhbox")
% «.bgcolorhbox»		(to "bgcolorhbox")
% «.firstcol-anothercol»	(to "firstcol-anothercol")
% «.co»				(to "co")
% «.ifundefined»		(to "ifundefined")
% «.cells»			(to "cells")


\def\N{\mathbb{N}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}


% «categories»  (to ".categories")
%
\def\Set {\mathbf{Set}}
\def\Sets{\mathbf{Sets}}
\def\Cat {\mathbf{Cat}}
\def\Grp {{\bf Grp}}
\def\Mon {{\bf Mon}}
\def\PTop{{\bf PTop}}
\def\Top {{\bf Top}}
\def\Vect{{\bf Vect}}
%
\def\catA{\mathbf{A}}
\def\catB{\mathbf{B}}
\def\catC{\mathbf{C}}
\def\catD{\mathbf{D}}
\def\catE{\mathbf{E}}
\def\catF{\mathbf{F}}
\def\catH{\mathbf{H}}
\def\catI{\mathbf{I}}
\def\catJ{\mathbf{J}}
\def\catP{\mathbf{P}}
%\def\OX{{\mathcal{O}_X}}
%\def\E{\mathbf{E}}
%\def\T{\mathbf{T}}
%\def\SetI{{\Set^{\mathbb{I}}}}
%\def\SetF{{\Set^{\mathcal{F}}}}
%\def\SetU{{\Set^{\mathcal{U}}}}
%\def\SetP{{\Set^{\mathbf{P}}}}
%\def\SetM{{\Set^{\mathbf{M}}}}
%\def\SetC{{\Set^{\bf C}}}
\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbP{\mathbb{P}}
\def\bbH{\mathbb{H}}
\def\bbV{\mathbb{V}}





% Quantificadores,
%
\def\Ex{\exists}
\def\Fa{\forall}
%\def\Exob#1{\mathop{\exists\;{#1}}}
%\def\Exbangob#1{\mathop{\exists!\;{#1}}}
%\def\Faob#1{\mathop{\forall\;{#1}}}
%\def\Exbang{\exists!}

\def\void {\varnothing}
\def\bsl  {\backslash}
\def\False{\Finv}
\def\nat  {\natural}



% «greek-letters»  (to ".greek-letters")
%
\def\aa{\alpha}
\def\bb{\beta}
\def\cc{\gamma}
\def\dd{\delta}
%\def\ee{\epsilon}
\def\ee{\varepsilon}    % (find-texbookpage (+ 12 128) "\\varepsilon")
\def\gg{\gamma}
\def\kk{\kappa}
\def\ww{\omega}
\def\Om{\Omega}
\def\Th{\Theta}
\def\GG{\Gamma}
\def\DD{\Delta}
\def\LL{\Lambda}
%
% (find-es "tex" "varphi")
%\let\origphi=\phi
%\def\phi{\varphi}

\def\superscriptOne  {^1}
\def\superscriptTwo  {^2}
\def\superscriptThree{^3}



\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calL{\mathcal{L}}
\def\calN{\mathcal{N}}
\def\calR{\mathcal{R}}
\def\calV{\mathcal{V}}



\def\id   {\mathrm{id}}
\def\ev   {\mathrm{ev}}
\def\cur  {\operatorname{\textsf{cur}}}
\def\uncur{\operatorname{\textsf{uncur}}}
\def\app  {\operatorname{app}}

\def\compr{\operatorname{compr}}
\def\Int  {\operatorname{Int}}

\def\adj   {\operatorname{adj}}

\def\hom   {\operatorname{hom}}
\def\Hom   {\operatorname{Hom}}
\def\op    {{\operatorname{op}}}
\def\colim {{\operatorname{colim}}}
\def\Colim {{\operatorname{Colim}}}
\def\Lim   {{\operatorname{Lim}}}
\def\src   {\operatorname{src}}
\def\tgt   {\operatorname{tgt}}
\def\dom   {\operatorname{dom}}
\def\cod   {\operatorname{cod}}
\def\Cod   {\operatorname{Cod}}
\def\Sub   {\operatorname{Sub}}
\def\CanSub{\operatorname{CanSub}}
\def\Objs  {\operatorname{Objs}}

\def\Props {\operatorname{Props}}
\def\Prfs  {\operatorname{Prfs}}
\def\prf   {\operatorname{prf}}

\def\fv     {\operatorname{fv}}
\def\FV     {\operatorname{FV}}
\def\welldef{{\operatorname{wd}}}
\def\welld  {{\operatorname{wd}}}




\def\setof    #1{\{\,#1\,\}}
\def\setofst#1#2{\{\,#1\;|\;#2\,\}}
\def\setofsc#1#2{\{\,#1\;;\;#2\,\}}
\def\Pts        {\mathcal{P}}



\def\ovl{\overline}

\def\nameof#1{\ulcorner#1\urcorner}
%
% (find-es "tex" "llangle-and-rrangle")
% (find-es "tex" "llbracket-and-rrbracket")
%
\def\llangle{\langle\!\langle}
\def\rrangle{\rangle\!\rangle}
\def\ang #1{\langle #1 \rangle}
\def\angg#1{\llangle#1\rrangle}
\def\angc  {\ang{\,,}}
%\def\<{\langle}
%\def\>{\rangle}
%
% Bananas
\def\ban#1{(\mskip-1.2\thinmuskip| #1 |\mskip-1.2\thinmuskip)}







% Calculus:
\def\sen   {\operatorname{sen}}
\def\arcsen{\operatorname{arcsen}}
\def\sec   {\operatorname{sec}}
\def\arcsec{\operatorname{arcsec}}

\def\uu{\vec u}
\def\vv{\vec v}
\def\ww{\vec w}
\def\Vec#1{{\overrightarrow{#1}}}
\def\VEC#1{{\overrightarrow{(#1)}}}



% «combinators»  (to ".combinators")
%
\def\cbS{\mathbf{S}}
\def\cbK{\mathbf{K}}
\def\cbI{\mathbf{I}}
\def\cbP{\mathbf{P}}
\def\cbD{\mathbf{D}}
\def\cbV{\mathbf{V}}
\def\cbT{\mathbf{T}}
\def\cbF{\mathbf{F}}
\def\SKI{\mathbf{SKI}}


% «colors»  (to ".colors")
% Mainly for slides.
%
\long\def\ColorRed   #1{{\color{Red1}#1}}
\long\def\ColorViolet#1{{\color{MagentaVioletLight}#1}}
\long\def\ColorViolet#1{{\color{Violet!50!black}#1}}
\long\def\ColorGreen #1{{\color{SpringDarkHard}#1}}
\long\def\ColorGreen #1{{\color{SpringGreenDark}#1}}
\long\def\ColorGreen #1{{\color{SpringGreen4}#1}}
\long\def\ColorGray  #1{{\color{GrayLight}#1}}
\long\def\ColorGray  #1{{\color{black!30!white}#1}}
\long\def\ColorBrown #1{{\color{Brown}#1}}
\long\def\ColorBrown #1{{\color{brown}#1}}
\long\def\ColorOrange#1{{\color{orange}#1}}
\long\def\ColorBlack #1{{\color{black}#1}}

% «standout»  (to ".standout")
% See: (find-es "tex" "xcolor")
%      (find-es "tex" "xcolor" "fcolorbox")
\def\standout#1{\fcolorbox{red}{yellow}{#1}}


% «mystrut»  (to ".mystrut")
% (find-es "tex" "mathstrut")
\def\mystrut#1#2{{\setbox0=\hbox{} \ht0=#1 \dp0=#2 \box0}}


% «bhbox»  (to ".bhbox")
% See: (find-es "tex" "bhbox")
\def\smashedvrule#1#2#3{\vrule width#1 height#2 depth#3 \kern-#1}
\def\bhboxuppercolor{yellow}
\def\bhboxlowercolor{orange}
\def\bhboxm#1{\bhbox{$#1$}}
\def\bhbox #1{\hbox{\bhboxz{#1}}}
\def\bhboxz#1{%
    \setbox0\hbox{#1}%
    {\color{\bhboxuppercolor}{\smashedvrule{\wd0}{\ht0}{0pt}}}%
    {\color{\bhboxlowercolor}{\smashedvrule{\wd0}{0pt}{\dp0}}}%
    \box0%
  }

% «bgcolorhbox»  (to ".bgcolorhbox")
% See: (find-dednat6 "tug-slides.tex" "bgcolorhbox")
\def\bgcolorhbox#1#2{{%
  \setbox0\hbox{#2}%
  \setbox0\vbox{\vskip\fboxsep\box0\vskip\fboxsep}%
  \setbox0\hbox{\kern\fboxsep\box0\kern\fboxsep}%
  {\color{#1}{\smashedvrule{\wd0}{\ht0}{\dp0}}}%
  \box0%
  }}


% «firstcol-anothercol»  (to ".firstcol-anothercol")
% (find-es "tex" "firstcol-anothercol")
\def\colwidth{8cm}
\long\def\firstcol#1{\begin{minipage}[t]{\colwidth} #1 \end{minipage}}
\long\def\anothercol#1{\qquad\firstcol{#1}}

% «co»  (to ".co")
% (find-es "tex" "co")
% (find-es "tex" "poor-mans-code")
% \co: a low-level way to typeset code; a poor man's "\verb"
% It conflicts with the `\co' of Category Theory =(
\def\co#1{{%
  \def\%{\char37}%
  \def\\{\char92}%
  \def\^{\char94}%
  \def\~{\char126}%
  \tt#1%
  }}
\def\qco#1{`\co{#1}'}
\def\qqco#1{``\co{#1}''}


% «ifundefined»  (to ".ifundefined")
% (find-es "tex" "ifundefined")
\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}


% «cells»  (to ".cells")
% (find-es "tex" "picture-cells")
% (find-es "tex" "ifx")
% (find-dn6 "preamble6.lua" "preamble1" "\\def\\cell")
\ifundefined  {celllower} \newlength {\celllower} \fi
\ifundefined {lcelllower} \newlength{\lcelllower} \fi
 \celllower=3pt    % For \documentclass[10pt]{...}
%\celllower=3.5pt  % For \documentclass[12pt]{...}

\def\cellfont{}
\def\lcellfont{}
\def\cell #1{\lower\celllower\hbox to 0pt{\hss\cellfont${#1}$\hss}}
\def\lcell#1{\lower\celllower\hbox to 0pt   {\lcellfont${#1}$\hss}}

% (find-es "tex" "ifx")
% (find-LATEX "material-para-GA.tex" "cells" "\\def\\cellnw")
\def\cellhr#1{\hbox to 0pt    {\cellfont${#1}$\hss}}
\def\cellhc#1{\hbox to 0pt{\hss\cellfont${#1}$\hss}}
\def\cellhl#1{\hbox to 0pt{\hss\cellfont${#1}$}}
\def\cellva#1{\setbox0#1\raise \dp0       \box0}
\def\cellvm#1{\setbox0#1\lower \celllower \box0}
\def\cellvb#1{\setbox0#1\lower \ht0       \box0}

\def\cellnw  #1{\cellva{\cellhl{#1}}}
 \def\celln  #1{\cellva{\cellhc{#1}}}
  \def\cellne#1{\cellva{\cellhr{#1}}}
\def\cellw   #1{\cellvm{\cellhl{#1}}}
 \def\celle  #1{\cellvm{\cellhr{#1}}}
\def\cellsw  #1{\cellvb{\cellhl{#1}}}
 \def\cells  #1{\cellvb{\cellhc{#1}}}
  \def\cellse#1{\cellvb{\cellhr{#1}}}

\ifundefined {cellsep} \newdimen\cellsep \fi
\cellsep=4pt
\def\addcellsep{%
  \setbox0=\hbox{\kern\cellsep\box0\kern\cellsep}%
  \ht0=\ht0 plus \cellsep%
  \dp0=\dp0 plus \cellsep%
  \box0%
}
\def\cellsp#1{%
  \setbox0=\hbox{#1}%
  \addcellsep%
  \box0%
}





\def\frown{\ensuremath{{=}{(}}}
\def\smile{\ensuremath{{=}{)}}}
\def\True {\mathbf{V}}
\def\False{\mathbf{F}}
\def\D    {\displaystyle}
\def\ph   {\phantom}


%\def\comp {\operatorname{comp}}

%\def\und#1{{\underline{#1}}}
% Often redefined to:
%\def\und#1#2{\underbrace{#1}_{#2}}














% Local Variables:
% coding:               utf-8-unix
% End:


==> edrxgac2.tex <==
% (find-angg "LATEX/edrxgac2.tex")
% edrxgac2: defs para Geometria Analítica e Cálculo 2
% Version: 2025feb02
% Usage:
%   \input edrxgac2.tex           % (find-angg "LATEX/edrxgac2.tex")
% See:                            % (find-angg "LATEX/edrxdefs.tex")

% «.GA»			(to "GA")
% «.matrices»		(to "matrices")
% «.C2»			(to "C2")
% «.C2-substnames»	(to "C2-substnames")
% «.pict2e»		(to "pict2e")
% «.beginpicture»	(to "beginpicture")
% «.pict-Vector»	(to "pict-Vector")
% «.verteq»		(to "verteq")



\def\R{\mathbb{R}}

\def\Rq{\ColorRed{?}}


%   ____    _    
%  / ___|  / \   
% | |  _  / _ \  
% | |_| |/ ___ \ 
%  \____/_/   \_\
%                
% «GA» (to ".GA")

% (find-LATEXfile "2015-2-GA-P1-gab.tex" "setofxyst")
% (find-LATEXfile "2015-1-GA-P2-gabarito.tex" "setxyst")
\def\nip{\par\noindent}
\def\uu{{\vec u}}
\def\vv{{\vec v}}
\def\ww{{\vec w}}
\def\Vec#1{\overrightarrow{#1}}
\def\VEC#1{{\overrightarrow{(#1)}}}
\def\Pr{{\text{Pr}}}
\def\Pru{\Pr_\uu}
\def\Prv{\Pr_\vv}
\def\Prw{\Pr_\ww}
\def\setofPst  #1{\setofst{P∈\R^2}{#1}}
\def\setofxyst #1{\setofst{(x,y)∈\R^2}{#1}}
\def\setofxyzst#1{\setofst{(x,y,z)∈\R^3}{#1}}
\def\setofexpron#1#2{\setofst{#1}{#2∈\R}}
\def\setofexprt#1{\setofst{#1}{t∈\R}}
\def\setofexpru#1{\setofst{#1}{u∈\R}}

\def\ii{{\vec i}}
\def\jj{{\vec j}}
\def\kk{{\vec k}}
\def\nn{{\vec n}}

% «matrices»  (to ".matrices")
% Shorthands for matrices
% (find-LATEXfile "2015planar-has.tex" "shorthand for matrices")
\def\mat #1{\begin       {matrix}#1\end{matrix}}
\def\pmat#1{\left (\begin{matrix}#1\end{matrix}\right )}
\def\bmat#1{\left [\begin{matrix}#1\end{matrix}\right ]}
\def\vmat#1{\left |\begin{matrix}#1\end{matrix}\right |}
\def\cmat#1{\left\{\begin{matrix}#1\end{matrix}\right\}}
\def\sm #1{\begin       {smallmatrix}#1\end{smallmatrix}}
\def\psm#1{\left (\begin{smallmatrix}#1\end{smallmatrix}\right )}
\def\bsm#1{\left [\begin{smallmatrix}#1\end{smallmatrix}\right ]}
\def\vsm#1{\left |\begin{smallmatrix}#1\end{smallmatrix}\right |}
\def\csm#1{\left\{\begin{smallmatrix}#1\end{smallmatrix}\right\}}

\def\mysubst#1{\bsm{#1}}

\def\area{\textsf{área}}
\def\Area{\textsf{Área}}
\def\Vol {\textsf{Vol}}



%   ____ ____  
%  / ___|___ \ 
% | |     __) |
% | |___ / __/ 
%  \____|_____|
%              
% «C2» (to ".C2")

\def\dydx{\frac{dy}{dx}}
\def\ddx {\frac{d}{dx}}
\def\ddth{\frac{d}{d\theta}}
\def\arcsen{\operatorname{arcsen}}
\def\sen{\operatorname{sen}}
\def\sec{\operatorname{sec}}
\def\ln{\operatorname{ln}}
%\def\ang{\operatorname{ang}}
\def\cosang{\operatorname{cos\ ang}}

\def\subst#1{\left[\sm{#1}\right]}

\def\veq{\rotatebox{90}{$=$}}
\def\mcc#1{\multicolumn{1}{c}{#1}}

\def\eqnpfull#1{\overset{\scriptscriptstyle(#1)}{=}}
\def\eqnpbare#1{=}
\def\eqnp      {\eqnpbare}
\def\qeqnp   #1{`$\eqnpfull{#1}$'}

\def\prims #1{∫#1\,ds}
\def\primth#1{∫#1\,dθ}


% Indefinite integrals
\def\ints    #1{∫#1\,ds}
\def\intc    #1{∫#1\,dc}
\def\intt    #1{∫#1\,dt}
\def\intu    #1{∫#1\,du}
\def\intv    #1{∫#1\,dv}
\def\intw    #1{∫#1\,dw}
\def\intx    #1{∫#1\,dx}
\def\inty    #1{∫#1\,dy}
\def\intz    #1{∫#1\,dz}
\def\intth   #1{∫#1\,dθ}
\def\intvar#1#2{∫#2\,d#1}

% Definite integrals
\def\Intr    #1#2#3{∫_{r=#1}^{r=#2}#3\,dr}
\def\Ints    #1#2#3{∫_{s=#1}^{s=#2}#3\,ds}
\def\Intt    #1#2#3{∫_{t=#1}^{t=#2}#3\,dt}
\def\Intu    #1#2#3{∫_{u=#1}^{u=#2}#3\,du}
\def\Intv    #1#2#3{∫_{v=#1}^{v=#2}#3\,dv}
\def\Intx    #1#2#3{∫_{x=#1}^{x=#2}#3\,dx}
\def\Inty    #1#2#3{∫_{y=#1}^{y=#2}#3\,dy}
\def\Intz    #1#2#3{∫_{z=#1}^{z=#2}#3\,dz}
\def\Intth   #1#2#3{∫_{θ=#1}^{θ=#2}#3\,dθ}
\def\Intvar#1#2#3#4{∫_{#1=#2}^{#1=#3}#4\,d#1}

% Difference
\def\difr    #1#2#3{\left. #3 \right|_{r=#1}^{r=#2}}
\def\difs    #1#2#3{\left. #3 \right|_{s=#1}^{s=#2}}
\def\dift    #1#2#3{\left. #3 \right|_{t=#1}^{t=#2}}
\def\difu    #1#2#3{\left. #3 \right|_{u=#1}^{u=#2}}
\def\difv    #1#2#3{\left. #3 \right|_{v=#1}^{v=#2}}
\def\difx    #1#2#3{\left. #3 \right|_{x=#1}^{x=#2}}
\def\difth   #1#2#3{\left. #3 \right|_{θ=#1}^{θ=#2}}
\def\difvar#1#2#3#4{\left. #4 \right|_{#1=#2}^{#1=#3}}

\def\Difs    #1#2#3{\left. #3 \right|_{s=#1}^{s=#2}}
\def\Difu    #1#2#3{\left. #3 \right|_{u=#1}^{u=#2}}
\def\Difv    #1#2#3{\left. #3 \right|_{v=#1}^{v=#2}}
\def\Difx    #1#2#3{\left. #3 \right|_{x=#1}^{x=#2}}
\def\Difth   #1#2#3{\left. #3 \right|_{θ=#1}^{θ=#2}}
\def\Difvar#1#2#3#4{\left. #4 \right|_{#1=#2}^{#1=#3}}

% «C2-substnames»  (to ".C2-substnames")
% \CSname{mainname}{addons}: color substitution name
% \CFname{mainname}{addons}: color formula name
% See: (c2m221dp1p 2 "introducao")
%      (c2m221dp1a   "introducao")
%      (find-es "tex" "xcolor" "green!40!yellow")
%      (find-xcolorpage 39 "4.4   Colors via x11names option")
%      (find-xcolortext 39 "4.4   Colors via x11names option")
\def\Sname #1#2{\ensuremath[\text{#1}#2]}
\def\CSname#1#2{{\color{Orange!80!red}\Sname{#1}{#2}}}
\def\CFname#1#2{{\ColorViolet{\Sname{#1}{#2}}}}
\def\CFname#1#2{{\color{SpringGreenDark}\Sname{#1}{#2}}}
\def\CFname#1#2{{\color{purple}\Sname{#1}{#2}}}
\def\CFname#1#2{{\color{Blue3}\Sname{#1}{#2}}}
\def\CFname#1#2{{\color{Red4}\Sname{#1}{#2}}}
\def\CFname#1#2{{\color{Red3}\Sname{#1}{#2}}}


\sa   {(*)}{\ensuremath{({*})}}
\sa  {(**)}{\ensuremath{({*}{*})}}
\sa {(***)}{\ensuremath{({*}{*}{*})}}
\sa{(****)}{\ensuremath{({*}{*}{*}{*})}}

\sa{*1}{\ensuremath{(*_1)}}
\sa{*2}{\ensuremath{(*_2)}}
\sa{*3}{\ensuremath{(*_3)}}
\sa{*4}{\ensuremath{(*_4)}}
\sa{*5}{\ensuremath{(*_5)}}
\sa{*6}{\ensuremath{(*_6)}}
\sa{*7}{\ensuremath{(*_7)}}




% «pict2e» (to ".pict2e")
% (find-LATEX "2016-2-C2-integral.tex" "pict2e")
% (find-LATEX "edrxpict.lua" "Piecewise")
% (find-LATEX "edrxpict.lua" "pictgrid")
% (find-LATEX "edrxpict.lua" "pictaxes")
% (find-LATEX "edrxpict.lua" "pictdots")

% «beginpicture» (to ".beginpicture")
% (find-LATEX "edrxpict.lua" "beginpicture")
% (find-es "tex" "begin-picture")
% (find-es "tex" "beginpicture")
\def\beginpicture (#1,#2)(#3,#4){\expr{beginpicture(v(#1,#2),v(#3,#4))}}
\def\beginpictureb(#1,#2)(#3,#4)#5{\expr{beginpicture(v(#1,#2),v(#3,#4),#5)}}

\def\pictaxes{\expr{pictaxes()}}
\def\pictaxes{{\linethickness{0.6pt}\expr{pictaxes()}}}
\def\pictaxes{{\linethickness{0.5pt}\expr{pictaxes()}}}
\def\pictgrid{{\color{GrayPale}\expr{pictgrid()}}}
\def\pictgrid{{\color{GrayPale}\linethickness{0.3pt}\expr{pictgrid()}}}
\def\pictdots#1{\expr{pictdots("#1")}}
\def\pictpiecewise#1{\expr{pictpiecewise("#1")}}
\def\pictpiecewise#1{{\linethickness{1pt}\expr{pictpiecewise("#1")}}}
\def\picturedots(#1,#2)(#3,#4)#5{%
  \vcenter{\hbox{%
  \beginpicture(#1,#2)(#3,#4)%
  \pictaxes%
  \pictdots{#5}%
  \end{picture}%
  }}%
}
\def\picturepiecewise(#1,#2)(#3,#4)#5{%
  \vcenter{\hbox{%
  \beginpicture(#1,#2)(#3,#4)%
  \pictgrid%
  \pictaxes%
  \pictpiecewise{#5}%
  \end{picture}%
  }}%
}

% \unitlength=9pt
\def\closeddot{\circle*{0.3}}
\def\opendot  {\circle*{0.3}\color{white}\circle*{0.2}}

% «pict-Vector» (to ".pict-Vector")
% (find-LATEX "edrxpict.lua" "pict2evector")
% (find-dn6 "picture.lua" "pict2e" "pict2evector =")
\def\Vector(#1,#2)(#3,#4){\expr{pict2evector(#1, #2, #3, #4)}}




% «verteq» (to ".verteq")
\def\verteq{
 \vcenter{\hbox{%
 \unitlength=1pt%
 \linethickness{0.4pt}%
 \beginpicture(0,0)(5,6)
   \roundcap
   \Line(1,0)(1,6)
   \Line(3,0)(3,6)
 \end{picture}%
 }}%
}



% (find-kopkadaly4page (+ 12 126) "\\parallel")
% (find-kopkadaly4text (+ 12 126) "\\parallel")
\def\myparallel{\mathop{{/}\!\!{/}}}







% Local Variables:
% ee-anchor-format: "«%s»"
% coding: utf-8-unix
% End:


==> edrxheadfoot.tex <==
% This file:
%   http://angg.twu.net/LATEX/edrxheadfoot.tex.html
%   http://angg.twu.net/LATEX/edrxheadfoot.tex
%           (find-angg "LATEX/edrxheadfoot.tex")
%             (find-es "tex" "edrxheadfoot.tex")
% Author: Eduardo Ochs <eduardoochs@gmail.com>
% Version: 2020sep14
% Public domain.
%
% I "\input" this file from most of my LaTeX files. It changes the
% code for headers and footers to make the page number appear in the
% header and the filename (the "\jobname", actually) and the date of
% the compilation appear of at the footer.
%
% (find-source2epage (+ 10 404) "64.1      Page Style Commands")
% (find-source2etext (+ 10 404) "64.1      Page Style Commands")
% (find-classespage 20 "\\ps@headings")
% (find-classestext 20 "\\ps@headings")
% (find-lsrcfile "base/article.cls")
% (find-lsrcfile "base/article.cls" "\\def\\ps@headings")
% (find-lsrcfile "base/book.cls")
% (find-lsrcfile "base/book.cls" "\\def\\ps@headings")
% (find-ldtxfile "base/classes.dtx")
% (find-ldtxfile "base/classes.dtx" "The page style")
% (find-ldtxfile "base/classes.dtx" "<!book>\\pagestyle{plain}")
% (find-kopkadaly4page (+ 12 335) "Page styles")
% (find-kopkadaly4text (+ 12 335) "Page styles")
%
\makeatletter
\newcount\m \newcount\n
\def\twodigits#1{\ifnum #1<10 0\fi \number#1}
\def\hours{\n=\time \divide\n 60
  \m=-\n \multiply\m 60 \advance\m \time
  \twodigits\n:\twodigits\m}
%
\def\draftfooter{\jobname{} \today{} \hours}
\def\footertext{\draftfooter}
\def\ps@headings{%
  \def\@oddfoot{\hfil \footertext \hfil}
  \let\@evenfoot\@oddfoot
  \def\@oddhead{{\slshape\rightmark}\hfil\thepage}%
  \let\@mkboth\markboth
  \def\chaptermark##1{%
    \markright {\MakeUppercase{%
      \ifnum \c@secnumdepth >\m@ne
        \if@mainmatter
          \@chapapp\ \thechapter. \ %
        \fi
      \fi
      ##1}}}}
\ps@headings
\makeatother
%
\def\shorttoday{%
  \number\year%
  \ifcase\month\or jan\or feb\or mar\or apr\or may\or
     jun\or jul\or aug\or sep\or oct\or nov\or dec\fi
  \twodigits\day}
\def\edrxnotesfooter#1{{\tiny #1 (typeset \shorttoday{} \hours)
  {\tt Edrx http://angg.twu.net/}}}
\def\edrxnotes#1{\gdef\footertext{\edrxnotesfooter{#1}}}
\def\noedrxfooter{\gdef\footertext{}}
%
% (find-es "tex" "edrxnotes")
% (find-fline "/usr/share/texmf-tetex/tex/generic/babel/portuges.ldf")
% (find-fline "/usr/share/texmf-tetex/tex/generic/babel/portuges.sty")


% Local Variables:
% coding:               utf-8-unix
% End:

